CARE: A Clue-guided Assistant for CSRs to Read User Manuals

It is time-saving to build a reading assistant for customer service representations (CSRs) when reading user manuals, especially information-rich ones. Current solutions don't fit the online custom service scenarios well due to the lack of attention to user questions and possible responses. Hence, we propose to develop a time-saving and careful reading assistant for CSRs, named CARE. It can help the CSRs quickly find proper responses from the user manuals via explicit clue chains. Specifically, each of the clue chains is formed by inferring over the user manuals, starting from the question clue aligned with the user question and ending at a possible response. To overcome the shortage of supervised data, we adopt the self-supervised strategy for model learning. The offline experiment shows that CARE is efficient in automatically inferring accurate responses from the user manual. The online experiment further demonstrates the superiority of CARE to reduce CSRs' reading burden and keep high service quality, in particular with >35% decrease in time spent and keeping a >0.75 ICC score.

==> Tables/ablation.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{Results of ablation study}
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
\textbf{Models}          & BLEU                           & Rouge-L                          & BERTScore                      \\ \hline
\sysname                     & \textbf{0.353}  & \textbf{0.497}  & \textbf{0.484}  \\ \hline
w/o beam search          & -0.013 & -0.010 & -0.015 \\ \hline
w/o joint inference & -0.034 & -0.022 & -0.034 \\ \hline
w/o heterogeneous model                  & -0.125 & -0.094 & -0.111 \\ \hline
\end{tabular}
}
\label{tab:ablation}
\end{table}

==> Tables/inference_algorithm.tex <==
\begin{algorithm}[t]
\small
        \renewcommand{\algorithmicrequire}{\textbf{Input:}}
        \renewcommand{\algorithmicensure}{\textbf{Output:}}
	\caption{Joint Inference Process} 
	\label{algorithm:infer}
        \begin{algorithmic}[1]

        \Require Graph $G = \{V, E\}$,  question clue node $n_{q} \in V $, link information $r$, threshold $\delta$, maximum inference depth $dep$; % input
        \Ensure Response clue nodes set $R$; % output

        % \State Define: $procedural\_path$ as edges linking actions in $G$, and $factual\_path$ as the remaining types of edges

        % \State Initialize threshold $\delta$
        % \State Initialize maximum inference depth $dep$
        \State $ R = \{\} $

        % \Function{Nei}{$n, \Phi$}
        % \State $path\_neighbors = set(); $
        %     \For{$n_{i} \in V$}
        %         \If{$n_{i} \in \Phi$}
        %             \State $path\_neighbors.add(n_{i})$
        %         \EndIf
        %     \EndFor
        % \State \Return $path\_neighbors$
            
        % \EndFunction

        \Function{Infer}{$n_{q}, r, \Phi$}
        \State \textbf{Initialize} $beam\_set = ( n_{q} ) $

        \While{$True$}
        
        \For{ $n_{j} \in beam\_set$ }
            \For{$n_{p} \in \Phi(n_{j})$}
                    \State update $beam\_set$ with \State $ \psi( n_{q}, r, n_{p} ) $ $\sim$ equation~\ref{equ:convr}
            \EndFor
        \EndFor
        
        \If{exist node $\geq \delta$}
            \State $R$.append$ ($top $n$ in $beam\_set$ $)$;
            \State break; 
        \EndIf
        
        \If{reach $dep$}
            \State $R$.append$ ($top $n$ in $beam\_set$ $)$;
            \State break; 
        \EndIf
        \EndWhile
            
        \EndFunction

        \State \texttt{INFER}($n_{q}, r, \mathbb{P}$)
        \State \texttt{INFER}($n_{q}, r, \mathbb{F}$)

        \State \Return $R$

\end{algorithmic}
\end{algorithm}

==> Tables/inference_algorithm_old.tex <==
\begin{algorithm}[t]
	\caption{Joint Inference on Constructed Graphs} 
	\label{algorithm:infer}
        \KwIn{Graph $G = \{V, E\}$,  question clue node $n_{q} \in V $, link information $r$ }
        \KwOut{Response clue nodes $\{ n_{r} \in V \}$ }
        \BlankLine

        Define: $procedural\_path$ as edges linking \\ actions in $G$, and $factual\_path$ as remaining \\ types of edges
        \BlankLine

        Initialize threshold $\delta$ \\
        Initialize maximum inference depth $dep$ \\
        output $ R = ( \  ) $ \\
        \BlankLine

        \SetKwFunction{Neighbors}{Neighbors}
        \SetKwProg{Fn}{Function}{:}{}
        \Fn{\Neighbors{ $n, path\_type$ }}{
            $path\_neighbors = set(); $ \\
            \ForEach{$n_{i} \in V$}{
                \If{$n_{i} \  and \  n \  are \  linked \  by \  path\_type$}{
                    $path\_neighbors.add(n_{i})$
                }
            }
            \Return $path\_neighbors$
        }

        \BlankLine

        \SetKwFunction{Infer}{Infer}
        \SetKwProg{Fn}{Function}{:}{}
        \Fn{\Infer{ $n_{q}, r, path\_type$ }}{
        \textbf{Initialize} $beam\_set = ( n_{q} ) $ \\ 
        
        \While{$True$}{
        
        \ForEach{ $n_{j}$ in $beam\_set$ }{
            \ForEach{$n_{p}$ in \textbf{Neighbors}( $n_{j}, path\_type$ )}{
                    update $beam\_set$ with \\ ConvR ( $n_{q}, r, n_{p}$ )
            }
        }
        \BlankLine
        
        \If{exist node $\geq \delta$}{
            $R$.append$ ($top $n$ in $beam\_set$ $)$; \\
            break; 
            }
        \If{reach $dep$}{
            $R$.append$ ($top $n$ in $beam\_set$ $)$; \\
            break; 
        }
        }
        
        }

        \BlankLine

        \textbf{Infer}($n_{q}, r, procedural\_path$)
        \textbf{Infer}($n_{q}, r, factual\_path$) \\
        
\end{algorithm}

==> Tables/main_results_old.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t]
\caption{Results of the offline experiment. The best performance results are highlighted \textbf{in bold}.}
\centering
\resizebox{\linewidth}{!}{
\begin{tabular}{l|c|c|c}
\hline
\textbf{Method}                 & BLEU                          & Rouge-L                         & BERTScore                     \\ \hline
\textbf{PERT}               & 0.100                       & 0.307                        & 0.251                        \\ \hline
\textbf{Fine-tuned PERT}    & {0.268}                  & {0.438}                  & 0.396                        \\ \hline
\textbf{TARA}                 & 0.199                          & 
0.361                        & 0.327                        \\ 
\hline
% \textbf{Heuristic KBQA}         & 0.0721                        & 0.1593                        & 0.1444                        \\ \hline
\textbf{DRGN}               & 0.209                        & 0.385                        & 0.356                         \\ \hline
\textbf{ChatGPT}                & 0.263                        & 0.418                        & {0.400}                  \\ \hline
\textbf{\sysname}                   & \textbf{0.353} & \textbf{0.497} & \textbf{0.484} \\ \hline
\end{tabular}
}
\label{tab:qa}
% \vspace{-0.5cm}
\end{table}


==> chapters/appx.tex <==
\appendix

\begin{figure*}[!th]
    \centering
    \subfigure[Co-reference Contents Highlighting]{\includegraphics[width=.45\textwidth]{case_fig/1.4.png}\label{fig:case1.4}}\hspace{1cm}
    \subfigure[Highlighting Specific Content]{\includegraphics[width=.45\textwidth]{case_fig/1.5.png}\label{fig:case1.5}}

    \vspace{1cm}
    \subfigure[Raw User Manual]{\includegraphics[width=.45\textwidth]{case_fig/1.1.png}\label{fig:case1.1}}\hspace{1cm}
    \subfigure[Response Only]{\includegraphics[width=.45\textwidth]{case_fig/1.2.png}\label{fig:case1.2}}

    \vspace{1cm}
    \subfigure[Clue-guided Assistant]{\includegraphics[width=.45\textwidth]{case_fig/1.3.png}\label{fig:case1.3}}
    
    \caption{An case of clues provided by different assistants for user question.}
    \label{fig:case1}
    \vspace*{-0cm}
\end{figure*}

\begin{figure*}[!th]
    \centering
    \subfigure[Co-reference Contents Highlighting]{\includegraphics[width=.45\textwidth]{case_fig/2.4.png}\label{fig:case2.4}}\hspace{1cm}
    \subfigure[Highlighting Specific Content]{\includegraphics[width=.45\textwidth]{case_fig/2.5.png}\label{fig:case2.5}}

    \vspace{1cm}
    \subfigure[Raw User Manual]{\includegraphics[width=.45\textwidth]{case_fig/2.1.png}\label{fig:case2.1}}\hspace{1cm}
    \subfigure[Response Only]{\includegraphics[width=.45\textwidth]{case_fig/2.2.png}\label{fig:case2.2}}\hspace{1cm}

    \vspace{1cm}
    \subfigure[Clue-guided Assistant]{\includegraphics[width=.45\textwidth]{case_fig/2.3.png}\label{fig:case2.3}}
    
    \caption{An case of clues provided by different assistants for inconsistent user questions.}
    \label{fig:case2}
    \vspace*{-0cm}
\end{figure*}

\clearpage

\section{Case Study}

Here we list some cases to demonstrate the superiority of our proposed assistant compared with other assistants. As shown in Figure~\ref{fig:case1}, for the question ``Where to set my nickname?'', the Co-reference Contents Highlighting approach highlights all the spans ``nickname'' in the manual and the Marking Specific Content approach highlights the ``kind tips'' section, both of them are nothing to do with the user question. Finally, our proposed assistant \name successfully locates the response ``personal profile page'' through in-depth inference on the procedural path. 

In more complex scenarios, as shown in Figure~\ref{fig:case2}, there is an inconsistency between the user question ``Why can't I apply for an international account?'' and corresponding manual, that is, specific action failure is not described directly in the user manual. The Co-reference Contents Highlighting approach can still only highlight all the spans ``Product Service'' which are useless for answering the question, and the Marking Specific Content approach even fails to match any spans. 
Unlike other assistants, our proposed assistant \name can conduct joint reference on both procedural and factual paths and successfully infers the procedural clue and factual clue for the failure of action ``apply for an international account'' mentioned in the question. This demonstrates that our proposed assistant can conduct in-depth inference on constructed graphs of manuals and is able to sufficiently locate potential responses through joint inference, further supporting CSRs in handling more complex user questions. 



\section{Details of the Constructed Graphs}
\label{graphs detail}
Here we provide a detailed introduction to the constructed graphs of user manuals and describe how can the model infer the desired clues of user questions on the graph through joint reasoning on both procedural and factual information. 

\begin{figure*}[!t]
    \centering
    \includegraphics[width=\textwidth]{figures/graph.png} 
    \caption{An example of the constructed graph.}
    \label{fig:graph}
     \vspace*{-0cm}
\end{figure*} 

\subsection{Graph Structure of User Manuals}
We construct user manuals into graphs as shown in Figure~\ref{fig:graph}. 
The graph consists of three kinds of nodes (i.e. action nodes, entity nodes, and argument nodes) and eight kinds of relations (i.e. Next, AGT, PAT, PATA, SUB, Action-ARG, Entity-ARG, and ARG-ARG). 
Firstly, the procedures containing a list of action nodes are constructed by linking actions belonging to the same procedure with the ``Next'' relation. 
We use the Next Sentence Prediction(NSP) of the pre-trained model~\cite{shi2019next} to determine whether two actions belong to the same procedure and construct all the procedures. 
To establish connections between agents and actions, we employ the "AGT" relation, while the "PAT" relation is utilized to connect patients with their respective actions. And the arguments of each action are linked through the ``Action-ARG'' relation, including the time, location, and manner description of the corresponding action. 
Secondly, we construct entity nodes and link their corresponding arguments through the ``Entity-ARG'' relation. The sub-entity of a certain entity is connected to it through a ``SUB'' relation. We also link the state of the entity with corresponding entities affected by it through the ``PATA'' relation and link the arguments associated with other entities' arguments through the ``ARG-ARG'' relation. 
Finally, We adopt character level matching to confirm the same entities and arguments references and fuse the same reference nodes into one node to avoid duplicate reference nodes of the constructed graphs. 

To support the heterogeneous inference of our proposed model, we retain the original three node types (e.g. ) and classify edge types into procedural and factual links. The former only includes the Next relationship in the graph, while the remaining relationships belong to factual link

\subsection{Response Clues Inference}
We construct the graphs of user manuals and adopt heterogeneous desired clues inference of user questions.
With the constructed graph, our proposed model can perform joint reasoning on both procedural and factual information for sufficient and robust inference. 
As shown in Figure~\ref{fig:graph}, to answer the user question ``Why can't I sign the policy?'', the model first needs to identify the core action ``sign'' that the user question is targeting as the question aligned node for subsequent inference of the desired clues. Starting from the question-aligned node, the model conducts in-depth reasoning on the graph of the manual to find potential clues to the user question. Through joint reasoning on both procedural and factual information, the model first refers to the previous action ``agree to'' of the aligned node through procedural meta-path based inference and finds the potential clue for the failure of the action ``sign'', that is the user did not complete the prerequisite operation ``agreeing to the insurance terms on the insurance application interface'', resulting in the inability to ``sign the policy''. Then the model further infers to the restrictions "Only real name authenticated users can participate in the insurance" associated with ``user'' node's sub-entity "real name authentication user" and ``User browsers that are not compatible with online signing tools may result in signing failure'' associated with ``user'' node's sub-entity ``user browser'' through factual meta-path based inference, which may also result in the failure of the action ``sign''. 
Through the constructed graph, our proposed model can perform joint reasoning on both procedural and factual information to find potential clues and guide CSRs to reach the responses to user questions. 

\section{Analysis of Generated Training Data}
\label{generated data analysis}

\begin{figure}[!ht]
    \centering
    \includegraphics[width=.98\textwidth]{figures/question_analysis.png}
    \caption{The top 10 actions and their top 4 patients of the questions in our generated training data.}
    \label{fig:question_analysis}
     % \vspace*{-0.5cm}
\end{figure}

% 43348  30670    4010 13.07 %  9.25%
To improve the generalization ability of the model, we strive to ensure the diversity of generated questions during the process of training data generation. We calculate the distribution of question types for the total 43348 samples we generated. We use the syntactic parsing tool~\cite{che2020n} to count the actions (verbs directly connected to the root in parsing trees) and corresponding patients (noun objects directly connected to the actions) in the generated questions. There are a total of 30670 questions with such a structure, while other factual style questions do not have such an ``action-patient'' structure (e.g. ``how much is the annual fee of membership benefits?''). We present the top 10 actions and their top 4 patients of the questions in our generated training data in Figure~\ref{fig:question_analysis}. We can see that the generated questions cover a wide range of actions, with a total of 4010 samples displayed, accounting for only 9.25\% of all generated questions and 13.07\% of all with an ``action-patient'' structure. 
For generated factual style questions, we take the connected entity nodes of the masked arguments as the question aligned nodes for self-supervised training. The labeled question aligned nodes can help identify the core concept of the question in the graph (e.g. the topic entity of the question existing in the graph). 
These generated factual style questions and procedural style questions involving diverse actions enhance the model's reasoning ability of desired clues for various questions raised by users in real-world scenarios and improve the generalization ability of the model. 

% \section{Experimental Details}
% \label{model detail}

% \subsection{Implementation Details}

